DocumentCLIP: Linking Figures and Main Body Text in Reflowed Documents

Vision-language pretraining models have achieved great success in supporting multimedia applications by understanding the alignments between images and text. While existing vision-language pretraining models primarily focus on understanding single image associated with a single piece of text, they often ignore the alignment at the intra-document level, consisting of multiple sentences with multiple images. In this work, we propose DocumentCLIP, a salience-aware contrastive learning framework to enforce vision-language pretraining models to comprehend the interaction between images and longer text within documents. Our model is beneficial for the real-world multimodal document understanding like news article, magazines, product descriptions, which contain linguistically and visually richer content. To the best of our knowledge, we are the first to explore multimodal intra-document links by contrastive learning. In addition, we collect a large Wikipedia dataset for pretraining, which provides various topics and structures. Experiments show DocumentCLIP not only outperforms the state-of-the-art baselines in the supervised setting, but also achieves the best zero-shot performance in the wild after human evaluation. Our code is available at https://github.com/FuxiaoLiu/DocumentCLIP.

==> Limitations.tex <==
In our Wikipedia dataset, we only have the section to image/caption linking as the groundtruth, which is automatically derived labels from layout cues (HTML labels). One potential solution is to have better data labeling – e.g. manually labeling all sentences according to image/text semantics, we can instead use a triplet-like loss that would allow for images to match to multiple sentences from different parts of the main body text. \cite{tran2020transform}'s dataset has the groundtruth linking between image/caption with sentences from articles. However, we don't have the right to use news articles according to the official website\footnote{https://help.nytimes.com/hc/en-us/articles/115014893428-Terms-of-Service#2}.
